Turbulent puffs in transitional pulsatile pipe flow at moderate pulsation amplitudes

We show that, in the transitional regime of pulsatile pipe flow, at moderate-to-high amplitudes 0.5 < A < 1, the first long-lived turbulent structures are localized and take the form of the puffs and slugs observed in statistically steady pipe flow. We perform direct numerical simulations at many pulsation frequencies, amplitudes and Re, and observe different dynamics of puffs and slugs. At certain flow parameters we find, using a causal analysis, that puffs actively make use of linear instabilities in the laminar Sexl-Womersley profile to survive the pulsation. Using all these lessons learned, we extend a low order model by Barkley et al., Nature (2015), to reproduce these dynamics. We find a good agreement between the extended model and our numerical results in a broad parametric space of pulsation amplitudes 0.5 < A < 1, frequencies Wo > 5 and 2100 < Re < 3000. With the help of our numerical results, causal analysis and model, we determine that turbulence production has two sources at these flow parameters: the mean shear as in statistically steady pipe flow, and the instabilities of the instantaneous pulsatile mean profile.

==> myPreamble.tex <==
% font encoding
\usepackage[utf8]{inputenc} % input
\usepackage[T1]{fontenc}    % output

\RequirePackage{siunitx}
\RequirePackage{xspace} % get your subsequent spacing straight
\DeclareRobustCommand{\ReTau}{\ensuremath{Re_{\tau}}\xspace}

\makeatletter
\def\oversortoftilde#1{\mathop{\vbox{\m@th\ialign{##\crcr\noalign{\kern3\p@}%
      \sortoftildefill\crcr\noalign{\kern3\p@\nointerlineskip}%
      $\hfil\displaystyle{#1}\hfil$\crcr}}}\limits}

\def\sortoftildefill{$\m@th \setbox\z@\hbox{$\braceld$}%
  \braceld\leaders\vrule \@height\ht\z@ \@depth\z@\hfill\braceru$}

\makeatother

\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amstext}
\RequirePackage{dsfont}
\PassOptionsToPackage{decimalsymbol=.}{siunitx}
\PassOptionsToPackage{binary-units=true}{siunitx}
\RequirePackage{siunitx}
\RequirePackage{xfrac}
\RequirePackage{booktabs}
\RequirePackage{tabularx}

% make it gay
\RequirePackage{xcolor}
\definecolor{Orange}{cmyk}{0, 0.5, 1, 0} % appropriate set for colour-blind
\definecolor{SkyBlue}{cmyk}{0.8, 0, 0, 0}
\definecolor{BluishGreen}{cmyk}{0.97, 0, 0.75, 0}
\definecolor{Yellow}{cmyk}{0.1, 0.05, 0.9, 0}
\definecolor{Blue}{cmyk}{1, 0.5, 0, 0}
\definecolor{Vermillion}{cmyk}{0, 0.8, 1, 0}
\definecolor{ReddishPurple}{cmyk}{0.1, 0.7, 0, 0}
\definecolor{Grey}{cmyk}{0, 0, 0, 0.6}
\definecolor{Black}{cmyk}{0, 0, 0, 1}

% math and stuff
\renewcommand{\vec}{\boldsymbol}
\DeclareRobustCommand{\increment}{\,d\hspace{-0.05em}}
\DeclareRobustCommand{\imag}{\ensuremath{\dot{\imath}}\xspace}  % imaginary unit
\DeclareRobustCommand{\real}{\ensuremath{\mathcal{R}}\xspace}   % real part
\DeclareRobustCommand{\orderof}{\ensuremath{O}\xspace}          % magnitude, JFM does NOT want \mathcal{O}
\DeclareRobustCommand{\ReTau}{\ensuremath{R\hspace{-0.1em}e_{\tau}}\xspace} % shear Reynolds number
\DeclareRobustCommand{\utau}{\ensuremath{u_{\tau}}\xspace}                  % friction velocity
\DeclareRobustCommand{\ubulk}{\ensuremath{u_{b}}\xspace}                    % bulk velocity
\DeclareRobustCommand{\Reynolds}{\ensuremath{R\hspace{-0.1em}e}\xspace}     % bulk Reynolds
\DeclareRobustCommand{\Womersley}{\ensuremath{W\hspace{-0.25em}o}\xspace}    % Womersley number
\DeclareRobustCommand{\Amplitude}{\ensuremath{A}\xspace}    % Amplitude
\DeclareRobustCommand{\ReDelta}{\ensuremath{R\hspace{-0.1em}e_{\delta}}\xspace} % Stokes layer Reynolds

\RequirePackage{hyperref}
\hypersetup{hidelinks}
\DeclareRobustCommand{\nsp}{\href{https://github.com/dfeldmann/nsCouette}{\textbf{\texttt{nsPipe}}}\xspace}
\DeclareRobustCommand{\opipe}{\href{https://openpipeflow.org/index.php?title=Main_Page}{\textbf{\texttt{openpipeflow}}}\xspace}
\DeclareRobustCommand{\pulsfor}{\href{https://pulseflow.uni-saarland.de}{\textbf{\texttt{Instabilities, Bifurcations and Migration in Pulsating Flow (FOR 2688)}}}\xspace}

% for draft stage only
%\usepackage[mathlines]{lineno}
%\linenumbers\relax
\RequirePackage{layouts}
\DeclareRobustCommand{\mod}[1]{{\color{Blue}#1}\xspace}
\DeclareRobustCommand{\modd}[1]{{\color{Blue}#1}\xspace}
\DeclareRobustCommand{\dm}[1]{{\color{Vermillion}(\textbf{DM}: \textit{#1})}\xspace}
\DeclareRobustCommand{\ma}[1]{{\color{Vermillion}(\textbf{MA}: \textit{#1})}\xspace}
\DeclareRobustCommand{\todo}[1]{{\color{Vermillion}(\textbf{To do}: \textit{#1})}\xspace}
\DeclareRobustCommand{\q}[1]{{\color{Vermillion}(\textbf{Question}: \textit{#1})}\xspace}

% averaging brackets
\DeclareRobustCommand{\lla}{\left\langle}
\DeclareRobustCommand{\rra}{\right\rangle}
